Machine Learning-Powered Course Allocation

We study the course allocation problem, where universities assign course schedules to students. The current state-of-the-art mechanism, Course Match, has one major shortcoming: students make significant mistakes when reporting their preferences, which negatively affects welfare and fairness. To address this issue, we introduce a new mechanism, Machine Learning-powered Course Match (MLCM). At the core of MLCM is a machine learning-powered preference elicitation module that iteratively asks personalized pairwise comparison queries to alleviate students' reporting mistakes. Extensive computational experiments, grounded in real-world data, demonstrate that MLCM, with only ten comparison queries, significantly increases both average and minimum student utility by 7%-11% and 17%-29%, respectively. Finally, we highlight MLCM's robustness to changes in the environment and show how our design minimizes the risk of upgrading to MLCM while making the upgrade process simple for universities and seamless for their students.

==> cover_letter.tex <==
Dear Editors,

We are pleased to submit the manuscript of our paper "Machine Learning-Powered Course Allocation" to be considered for publication in Management Science.

Abstract: We study the course allocation problem, where universities assign course schedules to students. The current state-of-the-art mechanism, Course Match, has one major shortcoming: students make significant mistakes when reporting their preferences, which negatively affects welfare and fairness. To address this issue, we introduce a new mechanism, Machine Learning-powered Course Match (MLCM). At the core of MLCM is a machine learning-powered preference elicitation module that iteratively asks personalized pairwise comparison queries to alleviate students' reporting mistakes. Extensive computational experiments, grounded in real-world data, demonstrate that MLCM, with only ten comparison queries, significantly increases both average and minimum student utility by 7%-11% and 17%-29%, respectively. Finally, we highlight MLCM's robustness to changes in the environment and show how our design minimizes the risk of upgrading to MLCM while making the upgrade process simple for universities and seamless for their students.


Our paper is situated at the intersection of market design and preference elicitation. Our ideal reviewers/AE would be experts in both of these areas and would appreciate an applied approach. For this reason, we would like to recommend Eric Budish from the University of Chicago Booth School of Business (eric.budish@chicagobooth.edu) as a Guest Associate Editor. We believe that Eric  would be exceptionally qualified to judge our paper given that he is the leading expert in course allocation. Budish et al. (Operations Research, 2017) introduced "Course Match", the current state-of-the-art course allocation mechanism. Budish et al. (EC, 2023) further improved the mechanism. Finally, Budish & Kessler (Management Science, 2022) studied how well Course Match is able to elicit students' preferences. Our work builds on all three of these papers.

Alternatively, we would like to recommend Peng Shi as an Associate Editor. Peng is an applied market designer with prior work on markets without money and experience with integrating prediction algorithms into allocation mechanisms. Finally, we would like to recommend Sasa Pecek as an Associate Editor. Sasa is an applied market designer with broad experience in optimization and statistical methods.


We would like to recommend the following five reviewers:
1) Eric Budish, in case he is not chosen as a Guest Associate Editor, for the reasons explained above.

2) Alex Teytelboym, who is an applied market designer with extensive experience in assignment problems. He has previously published in Management Science and he even has experience integrating machine learning into an allocation mechanism (Ahani et al., "Placement Optimization in Refugee Resettlement", Operations Research, 2021).

3) Alexey Kushnir, who is a versatile market designer. He has prior work on course allocation where, similar to our work, he uses a simulator based on real data to evaluate different course allocation mechanisms (Kornbluth and Kushnir, "Undergraduate Course Allocation through Competitive Markets", R&R at American Economic Review, 2023).

4) Thayer Morril, who is also a versatile market designer with prior work on course allocation (Bichler et al., "How to Assign Scarce Resources Without Money:  Designing Information Systems that are Efficient, Truthful, and (Pretty) Fair", Information Systems Research, 2021).

5) Ran Shorrer, who has multiple papers in applied market design for markets without money, including multiple papers published in Management Science.

Overall, none of the work presented in the manuscript we submit has been published before, and it is not currently under consideration for publication at any other journal. Please note that our manuscript is currently also under review at the 25th ACM Conference on Economic and Computation. In case the paper is accepted there, we will only publish a 1-page abstract in the EC proceedings.


We look forward to hearing from you.

Sincerely,
Sven Seuken

University of Zurich, Zurich
Binzmuhlestrasse 14, 8050 Zurich
seuken@ifi.uzh.ch



